Strictness of the Collapsible Pushdown Hierarchy

We present a pumping lemma for each level of the collapsible pushdown graph hierarchy in analogy to the second author's pumping lemma for higher-order pushdown graphs (without collapse). Using this lemma, we give the first known examples that separate the levels of the collapsible pushdown graph hierarchy and of the collapsible pushdown tree hierarchy, i.e., the hierarchy of trees generated by higher-order recursion schemes. This confirms the open conjecture that higher orders allow one to generate more graphs and more trees.

==> Chapter_Structure.tex <==
The proof of the pumping lemma consists of two parts.
In the first part (contained in Sections \ref{sec:BasicProp}-\ref{sec:types})
we define a function $\ctype$ which 
maps every configuration to a type. 
The image of $\ctype$ is finite and equipped with a partial order
$\typOrd$. 
The type of a configuration collects information about the existence
of certain runs starting in this configuration. 
Thus, for configurations $c_1, c_2$ with the same type, we can
transfer certain runs starting in $c_1$ to runs starting in $c_2$. 
The overall goal of the first part is to obtain the following three
transfer-properties.  

\begin{lemma}\label{lem:types1} 
  Let $R$ be a run of a CPS $\Ss$ such that
  $\hist{R}{\TOP{0}(R(\lvert R \rvert))}=\TOP{0}(R(0))$,  
  and let $c$ be a configuration such that $\ctype(R(0))\typOrd
  \ctype(c)$. 
  Then there exists a run $S$ from $c$ such that
  \begin{enumerate}
  \item	$\TOP0(R(|R|))=\TOP0(R(0))$ if and only if
    $\TOP0(S(|S|))=\TOP0(S(0))$, 
    % \item	the initial and the final stack of $R$ are the same if
    % and only if the initial and final stack of $S$ are the same, and 
  \item	$\hist{S}{\TOP{0}(S(\lvert S \rvert))}=\TOP{0}(c)$, 
  \item	all edges of $R$ are labelled by $\varepsilon$ if and only if
    all edges of $S$ are labelled by $\varepsilon$, and  
  \item	$\ctype(R(|R|))\typOrd \ctype(S(|S|))$. 
  \end{enumerate}
\end{lemma}

\begin{lemma}\label{lem:types2}
	Let $R$ be a run of a CPS $\Ss$ such that 
	some of its edges is not labelled by $\varepsilon$,
	and position $top^0(R(0))$ is present in every configuration of $R$.
	Let $c$ be a configuration such that $\ctype(R(0))\typOrd \ctype(c)$.
	Then there exists a run $S$ from $c$ such that 
	some of its edges is not labelled by $\varepsilon$,
	and position $top^0(c)$ is present in every configuration of $S$.
\end{lemma}

\begin{lemma}\label{lem:types3}
  Let $R$ be a run of a CPS $\Ss$, and let $c$ be a
  configuration such that $\ctype(R(0))\typOrd \ctype(c)$. 
  Then there exists a run $S$ from $c$ which ends in a
  configuration having the same state as $R(|R|)$. 
\end{lemma}

The second part of the proof uses these transfer properties in order
to proof the ``pumping lemma'' Theorem \ref{thm:pumping}. 
The proof strategy follows exactly the same lines as the proof of 
Parys' pumping lemma for higher-order pushdown systems (without
collapse) \cite{parys-panic-new}. We only have to adjust some minor
technical details. The proof can be found in Appendices
\ref{app:Combinatoric} and \ref{app:PumpingLemma}. 


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "Pumping-CPG"
%%% End: 

